Talk Less, Interact Better: Evaluating In-context Conversational Adaptation in Multimodal LLMs

Humans spontaneously use increasingly efficient language as interactions progress, by adapting and forming ad-hoc conventions. This phenomenon has been studied extensively using reference games, showing properties of human language that go beyond relaying intents. It remains unexplored whether multimodal large language models (MLLMs) similarly increase communication efficiency during interactions, and what mechanisms they may adopt for this purpose. We introduce ICCA, an automated framework to evaluate such conversational adaptation as an in-context behavior in MLLMs. We evaluate several state-of-the-art MLLMs, and observe that while they may understand the increasingly efficient language of their interlocutor, they do not spontaneously make their own language more efficient over time. This latter ability can only be elicited in some models (e.g., GPT-4) with heavy-handed prompting. This shows that this property of linguistic interaction does not arise from current training regimes, even though it is a common hallmark of human language. ICCA is available at https://github.com/lil-lab/ICCA.

==> figs/main_results/explicit_acc.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_llava_acc.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_Gemini_acc.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/explicit_consistency_acc.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_llava_acc.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_Gemini_acc.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/explicit_consistency_ed.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_IDEFICS_WND.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataidefics};
\label{plot:idefics_token}
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_llava_WND.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datallava};
\label{plot:llava_token}
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_GPT_WND.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datagpt};
\label{plot:gpt_token}
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_Gemini_WND.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datagemini};
\label{plot:gemini_token}
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_Claude_WND.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataclaude};
\label{plot:claude_token}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_WND.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datahuman};
\label{plot:human_token}
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/explicit_consistency_tokens.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_IDEFICS_tokens.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};

\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_llava_tokens.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};

\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_GPT_tokens.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};

\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_Gemini_tokens.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};

\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_Claude_tokens.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\label{plot:claude_token}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_tokens.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/explicit_consistency_wer.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_IDEFICS_WNR.csv}\dataIDEFICS
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataIDEFICS};
\addplot [name path=IDEFICSlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataIDEFICS};
\addplot [name path=IDEFICShigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataIDEFICS};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=IDEFICSlow and IDEFICShigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_llava_WNR.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_GPT_WNR.csv}\dataGPT
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataGPT};
\addplot [name path=GPTlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataGPT};
\addplot [name path=GPThigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataGPT};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=GPTlow and GPThigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_Gemini_WNR.csv}\dataGemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataGemini};
\addplot [name path=Geminilow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataGemini};
\addplot [name path=Geminihigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataGemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=Geminilow and Geminihigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicitconsistency_Claude_WNR.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_WNR.csv}\datahuman
\addhumanplottoken
table [x expr=\coordindex+2, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/explicit_ed.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_IDEFICS_WND.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataidefics};
\label{plot:idefics_token}
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_llava_WND.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datallava};
\label{plot:llava_token}
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_GPT_WND.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datagpt};
\label{plot:gpt_token}
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_Gemini_WND.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datagemini};
\label{plot:gemini_token}
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_Claude_WND.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataclaude};
\label{plot:claude_token}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_WND.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datahuman};
\label{plot:human_token}
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/explicit_tokens.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_IDEFICS_tokens.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};

\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_llava_tokens.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};

\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_GPT_tokens.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};

\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_Gemini_tokens.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};

\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_Claude_tokens.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\label{plot:claude_token}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_tokens.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/explicit_wer.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_IDEFICS_WNR.csv}\dataIDEFICS
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataIDEFICS};
\addplot [name path=IDEFICSlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataIDEFICS};
\addplot [name path=IDEFICShigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataIDEFICS};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=IDEFICSlow and IDEFICShigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_llava_WNR.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_GPT_WNR.csv}\dataGPT
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataGPT};
\addplot [name path=GPTlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataGPT};
\addplot [name path=GPThigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataGPT};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=GPTlow and GPThigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_Gemini_WNR.csv}\dataGemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataGemini};
\addplot [name path=Geminilow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataGemini};
\addplot [name path=Geminihigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataGemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=Geminilow and Geminihigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/explicit_Claude_WNR.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_WNR.csv}\datahuman
\addhumanplottoken
table [x expr=\coordindex+2, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/griceanhint_acc.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_llava_acc.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_Gemini_acc.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/griceanhint_ed.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_IDEFICS_WND.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataidefics};
\label{plot:idefics_token}
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_llava_WND.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datallava};
\label{plot:llava_token}
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_GPT_WND.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datagpt};
\label{plot:gpt_token}
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_Gemini_WND.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datagemini};
\label{plot:gemini_token}
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_Claude_WND.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataclaude};
\label{plot:claude_token}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_WND.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datahuman};
\label{plot:human_token}
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/griceanhint_tokens.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_IDEFICS_tokens.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};

\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_llava_tokens.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};

\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_GPT_tokens.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};

\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_Gemini_tokens.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};

\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_Claude_tokens.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\label{plot:claude_token}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_tokens.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/griceanhint_wer.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_IDEFICS_WNR.csv}\dataIDEFICS
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataIDEFICS};
\addplot [name path=IDEFICSlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataIDEFICS};
\addplot [name path=IDEFICShigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataIDEFICS};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=IDEFICSlow and IDEFICShigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_llava_WNR.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_GPT_WNR.csv}\dataGPT
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataGPT};
\addplot [name path=GPTlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataGPT};
\addplot [name path=GPThigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataGPT};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=GPTlow and GPThigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_Gemini_WNR.csv}\dataGemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataGemini};
\addplot [name path=Geminilow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataGemini};
\addplot [name path=Geminihigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataGemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=Geminilow and Geminihigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/griceanhint_Claude_WNR.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_WNR.csv}\datahuman
\addhumanplottoken
table [x expr=\coordindex+2, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/img_masked.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmasked_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmasked_llava_acc.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmasked_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmasked_Gemini_acc.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmasked_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/img_misleading.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmisleading_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmisleading_llava_acc.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmisleading_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmisleading_Gemini_acc.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgmisleading_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/imgonce.tex <==












\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgonce_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\label{plot:idefics}
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgonce_llava_acc.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\label{plot:llava}
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgonce_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\label{plot:gpt}
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgonce_Gemini_acc.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\label{plot:gemini}
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/imgonce_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\label{plot:claude}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\label{plot:human}
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/imgonce_misleadingRep6.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/misleadingRep6_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/misleadingRep6_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/misleadingRep6_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/no_hist.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/nohistory_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/nohistory_llava_acc.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/nohistory_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/nohistory_Gemini_acc.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/nohistory_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/no_shuffle.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/noshuffle_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/noshuffle_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];





\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/standard_speaker_acc.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_llava_acc.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_Gemini_acc.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_Claude_acc.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/standard_speaker_ed.tex <==














\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_IDEFICS_WND.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataidefics};
\label{plot:idefics_token}
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_llava_WND.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datallava};
\label{plot:llava_token}
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_GPT_WND.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datagpt};
\label{plot:gpt_token}
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_Gemini_WND.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datagemini};
\label{plot:gemini_token}
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_Claude_WND.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataclaude};
\label{plot:claude_token}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_WND.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datahuman};
\label{plot:human_token}
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/standard_speaker_tokens.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_IDEFICS_tokens.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\label{plot:idefics_token}
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_llava_tokens.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datallava};
\label{plot:llava_token}
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_GPT_tokens.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\label{plot:gpt_token}
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_Gemini_tokens.csv}\datagemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagemini};
\label{plot:gemini_token}
\addplot [name path=geminilow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagemini};
\addplot [name path=geminihigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=geminilow and geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_Claude_tokens.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataclaude};
\label{plot:claude_token}
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_tokens.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\label{plot:human_token}
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/standard_speaker_wer.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_IDEFICS_WNR.csv}\dataIDEFICS
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataIDEFICS};
\addplot [name path=IDEFICSlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataIDEFICS};
\addplot [name path=IDEFICShigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataIDEFICS};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=IDEFICSlow and IDEFICShigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_llava_WNR.csv}\datallava
\addplot [semithick, plotcolor4, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\datallava};
\addplot [name path=llavalow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datallava};
\addplot [name path=llavahigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datallava};
\addplot [fill=plotcolor4, opacity=0.2] fill between[of=llavalow and llavahigh];



\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_GPT_WNR.csv}\dataGPT
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataGPT};
\addplot [name path=GPTlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataGPT};
\addplot [name path=GPThigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataGPT};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=GPTlow and GPThigh];

   

\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_Gemini_WNR.csv}\dataGemini
\addplot [semithick, plotcolor11, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataGemini};
\addplot [name path=Geminilow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataGemini};
\addplot [name path=Geminihigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataGemini};
\addplot [fill=plotcolor11, opacity=0.2] fill between[of=Geminilow and Geminihigh];




\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardspeaker_Claude_WNR.csv}\dataclaude
\addplot [semithick, plotcolor12, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+2, y={y_values}]{\dataclaude};
\addplot [name path=claudelow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\dataclaude};
\addplot [name path=claudehigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\dataclaude};
\addplot [fill=plotcolor12, opacity=0.2] fill between[of=claudelow and claudehigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_WNR.csv}\datahuman
\addhumanplottoken
table [x expr=\coordindex+2, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+2, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+2, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];


==> figs/main_results/standardlistener.tex <==
\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardlistener_IDEFICS_acc.csv}\dataidefics
\addplot [semithick, plotcolor1, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\dataidefics};
\addplot [name path=ideficslow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\dataidefics};
\addplot [name path=ideficshigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\dataidefics};
\addplot [fill=plotcolor1, opacity=0.2] fill between[of=ideficslow and ideficshigh];

\pgfplotstableread[col sep=comma,]{figs/main_results/data/standardlistener_GPT_acc.csv}\datagpt
\addplot [semithick, plotcolor2, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datagpt};
\addplot [name path=gptlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datagpt};
\addplot [name path=gpthigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datagpt};
\addplot [fill=plotcolor2, opacity=0.2] fill between[of=gptlow and gpthigh];


\pgfplotstableread[col sep=comma,]{figs/main_results/data/Human_acc.csv}\datahuman
\addplot [semithick, plotcolor9, mark=*, mark size=1, mark options={solid}]
table [x expr=\coordindex+1, y={y_values}]{\datahuman};
\addplot [name path=humanlow, draw=none] table [x expr=\coordindex+1, y={ci_low}]{\datahuman};
\addplot [name path=humanhigh, draw=none] table [x expr=\coordindex+1, y={ci_high}]{\datahuman};
\addplot [fill=plotcolor9, opacity=0.2] fill between[of=humanlow and humanhigh];
\label{plot:human}


==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

